Implicit Neural Representation for Physics-driven Actuated Soft Bodies

Active soft bodies can affect their shape through an internal actuation mechanism that induces a deformation. Similar to recent work, this paper utilizes a differentiable, quasi-static, and physics-based simulation layer to optimize for actuation signals parameterized by neural networks. Our key contribution is a general and implicit formulation to control active soft bodies by defining a function that enables a continuous mapping from a spatial point in the material space to the actuation value. This property allows us to capture the signal's dominant frequencies, making the method discretization agnostic and widely applicable. We extend our implicit model to mandible kinematics for the particular case of facial animation and show that we can reliably reproduce facial expressions captured with high-quality capture systems. We apply the method to volumetric soft bodies, human poses, and facial expressions, demonstrating artist-friendly properties, such as simple control over the latent space and resolution invariance at test time.

==> script.tex <==
We present a physics- and data-driven method to control active soft bodies. Our implicit representation enables a continuous mapping from a spatial point in the material space to the control parameters, enabling shape invariance and hence general applicability to a wide range of soft body representations.

Using a set of observations, we learn actuation signals and mandible kinematics, such that when using these parameters in a forward pass, the simulation output matches ground truth.

We implicitly represent two mechanical properties using coordinate based neural networks and couple them with a differentiable soft body simulator to allow gradient information to flow from the solver to the networks. The encoder is a global shape descriptor complemented with a resolution value and outputs a latent code.

Here we show our training datasets such as synthetic starfish, a dancing sequence from AMASS and a facial performance dataset.

In all examples, our trained models can reliably reproduce target shapes with the optimized parameters, as indicated by low reconstruction error. 

The actuation signals are color coded on the hexahedral mesh. Note that the network contains less than three hundred thousand parameters but has excellent representational power for fine detail reconstructions such as wrinkles.

For the face, we optimized both actuation signals and mandible kinematics. 
Thanks to the jaw generative network, we can directly compute a jaw position that is compatible with the actuation.

With our trained model, we can fit new expressions by keeping the weights of neural networks fixed and optimizing for the latent code that yields the best fit. This sequence shows the result for unseen target poses and the associated low errors.

We interpolate between nine expressions, indicating smooth transitions despite the non-linearity of the deformation. The actuation and jaw position are also consistently interpolated.

Our method successfully generalizes to continuous resolution input. The resolution invariance property paves the way for efficient practical use where the resolution can be chosen at test time depending on the requirements at hand.

Transfer learning can be used as an alternative strategy to the proposed continuous resolution approach. It requires only one epoch to make the network consistent with the new discretization. 

Our results indicate that the trained model can accurately represent the dominant frequencies of the actuation signal and reproduce them at test time.

We compared our method with blendshapes. The error maps show clearly the superiority of our method, which can be accounted to the non-linearity of our model.

Lastly, we show the necessity of our normal constraint in the loss function for the face example. The normal constraint positively affects the fidelity of the resulting wrinkles and facial details.

Thanks for watching.
